Control-Flow Residual Analysis for Symbolic Automata

Where full static analysis of systems fails to scale up due to system size, dynamic monitoring has been increasingly used to ensure system correctness. The downside is, however, runtime overheads which are induced by the additional monitoring code instrumented. To address this issue, various approaches have been proposed in the literature to use static analysis in order to reduce monitoring overhead. In this paper we generalise existing work which uses control-flow static analysis to optimise properties specified as automata, and prove how similar analysis can be applied to more expressive symbolic automata - enabling reduction of monitoring instrumentation in the system, and also monitoring logic. We also present empirical evidence of the effectiveness of this approach through an analysis of the effect of monitoring overheads in a financial transaction system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{29}
\providecommand{\publicationstatus}{Adrian Francalanza, Gordon J. Pace (Eds.): Second International Workshop\\
on Pre- and Post-Deployment Verification Techniques (PrePost 2017)\\
EPTCS 254, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.254.3}{10.4204/EPTCS.254.3}}

